Mood Classification of Bangla Songs Based on Lyrics

Music can evoke various emotions, and with the advancement of technology, it has become more accessible to people. Bangla music, which portrays different human emotions, lacks sufficient research. The authors of this article aim to analyze Bangla songs and classify their moods based on the lyrics. To achieve this, this research has compiled a dataset of 4000 Bangla song lyrics, genres, and used Natural Language Processing and the Bert Algorithm to analyze the data. Among the 4000 songs, 1513 songs are represented for the sad mood, 1362 for the romantic mood, 886 for happiness, and the rest 239 are classified as relaxation. By embedding the lyrics of the songs, the authors have classified the songs into four moods: Happy, Sad, Romantic, and Relaxed. This research is crucial as it enables a multi-class classification of songs' moods, making the music more relatable to people's emotions. The article presents the automated result of the four moods accurately derived from the song lyrics.

==> sn-bibliography.bib.tex <==

@book{bib1,
  title={Neuromarketing: Exploring the brain of the consumer},
  author={Zurawicki, Leon},
  year={2010}
}
@article{bib2,
  title={Current challenges and visions in music recommender systems research},
  author={Schedl, Markus and Zamani, Hamed and Chen, Ching-Wei and Deldjoo, Yashar and Elahi, Mehdi},
  journal={International Journal of Multimedia Information Retrieval},
  volume={7},
  pages={95--116},
  year={2018},
  publisher={Springer}
}
@article{bib3,

  title={Social pleasures of music},
  author={Nummenmaa, Lauri and Putkinen, Vesa and Sams, Mikko},
  journal={Current Opinion in Behavioral Sciences},
  volume={39},
  pages={196--202},
  year={2021},
  publisher={Elsevier}
}
  
@inproceedings{bib4,
  title = {MuseBERT: Pre-training Music Representation for Music Understanding and Controllable Generation},
  author = {Ziyu Wang and Gus Xia},
  year = {2021},
  researchr = {https://researchr.org/publication/0008X21-0},
  cites = {0},
  citedby = {0},
  pages = {722-729},
  booktitle = {22nd International Society for Music Information Retrieval Conference, ISMIR 2021, Online, November 7-12, 2021},
  editor = {Jin Ha Lee 0001 and Alexander Lerch 0001 and Zhiyao Duan and Juhan Nam and Preeti Rao and Peter van Kranenburg and Ajay Srinivasamurthy},
  isbn = {978-1-7327299-0-2},
}
@article{bib5,
  author		= "Walaa Medhat, Ahmed Hassan, Hoda Korashy",
  title			= "Sentiment analysis algorithms and applications: A survey",
  journal		= " Ain Shams Engineering Journal",
  volume		= "5",
  Issue		= "4",
  pages			= "1093-1113",
  year			= "2014",
%  doi   ="10.1016/j.asej.2014.04.011"
}

%% Journal article with DOI
@article{bib6,
  author		= "Doaa Mohey El-Din Mohamed Hussein,",
  title			= "A survey on sentiment analysis challenges,",
  journal		= "Journal of King Saud University - Engineering Sciences,",
  volume		= "30",
  pages			= "330-338",
  year			= "2018",
%  doi			= "10.1016/j.jksues.2016.04.002"
}
%% book, authored
@book{bib7,
  author		= "Rabeya, Tapasy and Chakraborty, Narayan Ranjan and Ferdous, Sanjida and Dash, Manoranjan and Al Marouf, Ahmed",
  booktitle="2019 IEEE International Conference on Electrical, Computer and Communication Technologies (ICECCT)",
  title			= "Sentiment Analysis of Bangla Song Review- A Lexicon Based Backtracking Approach",
  year			= "2019",
  pages = "1-7",
%  doi={10.1109/ICECCT.2019.8869290}
}
@article{bib8,
  title={Bangla Music Genre Classification Using Neural Network},
  author={Md. Afif Al Mamun and Imam Abdul Kadir and AKM SHAHARIAR AZAD RABBY and Abdullah Al Azmi},
  journal={2019 8th International Conference System Modeling and Advancement in Research Trends (SMART)},
  year={2019},
  pages={397-403}
}
@inproceedings{bib9,
author = {Zaanen, Menno and Kanters, Pieter},
year = {2010},
month = {01},
pages = {75-80},
title = {Automatic Mood Classification Using TF*IDF Based on Lyrics.},
journal = {Proceedings of the 11th International Society for Music Information Retrieval Conference, ISMIR 2010}
}
@inproceedings{bib10,
author = {Kashyap, Nirbhay and Choudhury, Tanupriya and Chaudhary, Dev and Lal, Roshan},
year = {2016},
month = {09},
pages = {287-292},
title = {Mood Based Classification of Music by Analyzing Lyrical Data Using Text Mining},

}
@article{bib11,
  title={MusicMood: Predicting the mood of music from song lyrics using machine learning},
  author={S. Raschka},
  journal={ArXiv},
  year={2016},
  volume={abs/1611.00138}
}
@inbook{bib12,
author = {Urmi, Nazia and Ahmed, Nasir and Sifat, Md.Habibur and Islam, Salekul and Jameel, Abu},
year = {2021},
month = {01},
pages = {673-681},
title = {BanglaMusicMooD: A Music Mood Classifier from Bangla Music Lyrics},
isbn = {978-3-030-49794-1},
%doi = {10.1007/978-3-030-49795-8_64}
}

@inproceedings{bib13,
  title={Music Mood Dataset Creation Based on Last.fm Tags},
  author={Erion Çano and Maurizio Morisio},
  year={2017}
}
@article{bib14,
  title={BERT: Pre-training of Deep Bidirectional Transformers for Language Understanding},
  author={Jacob Devlin and Ming-Wei Chang and Kenton Lee and Kristina Toutanova},
  journal={ArXiv},
  year={2019},
  volume={abs/1810.04805}
}
@INPROCEEDINGS{bib15,
  author={Kaliyar, Rohit Kumar},
  booktitle={2020 10th International Conference on Cloud Computing, Data Science & Engineering (Confluence)}, 
  title={A Multi-layer Bidirectional Transformer Encoder for Pre-trained Word Embedding: A Survey of BERT}, 
  year={2020},
  volume={},
  number={},
  pages={336-340}
}
@article{bib16,
  title={Huggingface's transformers: State-of-the-art natural language processing},
  author={Wolf, Thomas and Debut, Lysandre and Sanh, Victor and Chaumond, Julien and Delangue, Clement and Moi, Anthony and Cistac, Pierric and Rault, Tim and Louf, R{\'e}mi and Funtowicz, Morgan and others},
  journal={arXiv preprint arXiv:1910.03771},
  year={2019}
}
@article{bib17,
author = {Chi, Sun and Qiu, Xipeng and Xu, Yige and Huang, Xuanjing},
year = {2019},
month = {05},
pages = {},
title = {How to Fine-Tune BERT for Text Classification?}
}

